Learning to be Safe: Deep RL with a Safety Critic

Safety is an essential component for deploying reinforcement learning (RL) algorithms in real-world scenarios, and is critical during the learning process itself. A natural first approach toward safe RL is to manually specify constraints on the policy's behavior. However, just as learning has enabled progress in large-scale development of AI systems, learning safety specifications may also be necessary to ensure safety in messy open-world environments where manual safety specifications cannot scale. Akin to how humans learn incrementally starting in child-safe environments, we propose to learn how to be safe in one set of tasks and environments, and then use that learned intuition to constrain future behaviors when learning new, modified tasks. We empirically study this form of safety-constrained transfer learning in three challenging domains: simulated navigation, quadruped locomotion, and dexterous in-hand manipulation. In comparison to standard deep RL techniques and prior approaches to safe RL, we find that our method enables the learning of new tasks and in new environments with both substantially fewer safety incidents, such as falling or dropping an object, and faster, more stable learning. This suggests a path forward not only for safer RL systems, but also for more effective RL systems.

==> Learning to be Safe - Arxiv/1-introduction.tex <==

%%CF.1.18: In general, this is written quite well. But, I think this story if perhaps too focused on the curriculum aspect and less on the learning safety aspect. Here's one way we could include the latter: 
While reinforcement learning systems have demonstrated impressive potential in a variety of domains, including video games~\cite{Mnih2013PlayingAW} and robotic control in laboratory environments~\cite{levine2015end}, safety remains a critical bottleneck when deploying these systems for real world problems. One natural approach to ensure safety is to manually impose constraints onto the learning process, to prevent the agent from taking actions or entering states that are too risky. For example, this could be done by manually shaping a reward function or imposing constraints on the policy to avoid actions that may lead to unsafe outcomes~\cite{45450}. 
%%CF.1.26: Can we add citations to a couple more additional works here?
% However, the success of machine learning techniques in a breadth of fields has taught us the pitfalls of manual engineering and specification, particularly in diverse open-world environments 
However, the recent successes of machine learning techniques in a wide range of applications indicate advantages to avoiding manual specification and engineering, as such manual approaches will not generalize to new environments or robots~\cite{robonet}. This begs the question: why should we make an exception with safety? In this paper, we propose to explore the following question: can we \emph{learn} how to be safe, avoiding the need to manually specify states and actions that are risky?


% TODO: change Q_safe to Q_safe^\pibar
% TODO: finetuneing phase, learning pi^* for the given new task instance, s.t. Q_safe^pibar < eps 
% DONE
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{Figures/fig1.pdf}
    \vspace{-0.1cm}
    \caption{Our approach enables safe RL by pre-training a critic $Q_\text{safe}^{\bar{\pi}}$ that is trained by constraining the actions of a policy $\pi$. This yields safe policy iterates (resulting from optimizing Eq.~\ref{eq:pol-ft}) that achieve safe episodes throughout fine-tuning, while standard RL approaches will visit unsafe states during adaptation, which results in more failed episodes.}
    \label{fig:hand-safe}
    \vspace{-1em}
\end{figure*}

% 2nd paragraph: Learning and safety may seem inherently at odds. However, when children learn to walk, ...
At first, learning and safety may seem inherently at odds, since learning to be safe requires visiting unsafe states. However, when children learn to walk they can leverage the positive and negative experience of getting up and falling down to gradually begin to stand, walk, and eventually run. Throughout this process, they learn how to move around in the world safely and adapt these skills as their bodies grow and are exposed to new and unseen environments, all while limiting how badly and often they are injured. This way of safely exploring while learning is something that can not only be used when learning to walk, but in other areas where safety is critical not only for survival, but generally helpful for successfully learning the task.
% For instance, after learning how to avoid colliding into objects or falling down, it can be safer and easier to learn new skills such as ice-skating or driving.
For instance, an agent can more safely learn to drive a car if it already knows how to avoid collisions.


%%CF.1.18: You took a bit of a jump in the last sentence. Can you break it down a bit? e.g. "where safety is critical not only for survival, but also helpful for successfully learning the task."

%%CF.1.18: At this stage, we need to make it clear what we're proposing. One way to do that would be to replace the next two paragraphs with:

Motivated by how humans learn to acquire skills that become gradually harder and more risky, we believe that our reinforcement learning agents can similarly leverage previous experience to understand general safety precautions in safety-training environments, and use this understanding to avoid failures when learning \emph{new behaviors}. This previous experience could come from non-safety-critical environments such as when a human is present, when a robot is moving slowly, in simulation, or from pre-collected offline data of safety incidents such as car accidents.  To this end, we propose to learn task-agnostic models of safety, and then use these models such as preventing unsafe behavior when learning new tasks via reinforcement. By doing so, we can ensure that the latter reinforcement learning process itself is safe, which in principle, can enable real-world deployment. 
%%CF.1.23: The below doesn't at all flow in this paragraph, so I'm commenting it out.
%Similarly, in various robotics domains, we may want to develop learning algorithms that not only teach a robot to solve a difficult task, but additionally teach it to gradually learn how to be safe. For instance, we may want it to learn general safety precautions and principles that can generalize to various other domains or more difficult task instances, and know not to repeat mistakes that have already been made during training on other tasks.

% We consider the problem of learning a task-agnostic safety model which can evaluate whether a given state, action pair will lead to an unsafe state in the future. This model should be learned rather than enforced through fixed constraints so that it can be robust to unobserved changes in the environment dynamics across different tasks. Using a fixed model that is designed for a specific task instance may not work well under a new setting. Furthermore, we are interested in whether this model can be useful in learning to perform new tasks more quickly, while also limiting the cumulative safety regret during training, which is the aggregate number of times the agent reaches an unsafe state.

%%CF.1.18: With my above rephrasing, this paragraph could start more along the lines of "The primary contribution of this work is a framework for incrementally safe reinforcement learning. Our approach, safety Q-functions for reinforcement learning (SQRL), learns whether a state, action pair will lead to unsafe behavior under a policy that is constrained by the safety model itself. [a sentence about how we pre-train and fine-tune / learn incrementally] We evaluate our method on three domains: ...
%%CF.1.23: I made some revisions to the below
The primary contribution of this work is a framework for safe reinforcement learning, by learning safety precautions from previous experience. Our approach, safety Q-functions for reinforcement learning (SQRL), learns a critic that evaluates whether a state, action pair will lead to unsafe behavior, under a policy that is constrained by the safety-critic itself. This is achieved by concurrently training the safety-critic and policy in separate pre-training and task fine-tuning phases, visualized in Figure~\ref{fig:hand-safe}. During pre-training, the agent is allowed to explore and learn about unsafe behaviors. In the fine-tuning phase, we train the policy on a new target task, while simultaneously constraining the policy's updates and selected actions with the safety-critic. We evaluate our method in three challenging continuous control environments: 2D navigation, quadrupedal robot locomotion, and dexterous manipulation with a five-fingered hand. In comparison to prior state-of-the-art RL methods and approaches to safety, we find that SQRL provides consistent and substantial gains in terms of both the safety of learning and the learning efficiency on new tasks.

%%CF.1.18: toy point-mass environment -> 2D navigation
%%CF.1.18: it -> method name
%%CF.1.18: Be more specific, and don't call them baselines. Some of them are SOTA prior methods, and baselines understates how strong they are.
%%CF.1.18: cite SAC if you're going to mention it.
%%CF.1.18: I don't think it will be clear what you mean by this.

%%CF.1.18: A teaser figure would be good to include. There are a couple options we could do here:
% One option would be to focus on the empirical results; for example, a one or two column figure that shows exploration on the minitaur and shadow hand without safety incidents (e.g. with a caption that says "Our approach enables a quadruped to learn to run faster while only falling X times in the learning process, and a five fingered hand to rotate a cube to a new position while only dropping the cube X times." Could also replace X with a percentage compared to standard RL)
% Another option would be to focus on communicating the method, while still including pictures of the minitaur or hand. (see this paper for an example of this: https://arxiv.org/abs/1603.00448)

\iffalse
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\linewidth]{Figures/teaser.pdf}
\caption{A visualization of how actions are filtered according to their probability of causing a safety incident.}
\end{figure}
\fi

% \begin{figure}[t!]
 
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.8\linewidth]{drunk_spider} 
% \caption{Drunk Spider environment and possible paths to the goal}
% \label{fig:ds}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.8\linewidth]{minitaur}
% \caption{PyBullet Minitaur environment}
% \label{fig:minitaur}
% \end{subfigure}
% \caption{Multi-task environments used in our experiments}
% \label{fig:envs}
% \end{figure}


==> Learning to be Safe - Arxiv/2-related.tex <==
%%CF.1.18: When you write a related work section, you shouldn't explain what every work does. The important thing to do is to explain the most salient differences between your work and the prior works. To do this effectively, I would recommend grouping papers together based on a relevant common denominator. An example of a good related work section is this one: https://arxiv.org/pdf/1912.03820.pdf

% Here is some guidance on how it could be structured:
% First paragraph can start with the basics: "Our work builds on a rich body of work on safe reinforcement learning~\cite{safe_rl_survey}. Prior works have defined safety in a range of ways, including constraints on the expected value~\cite{x,y,z,constrained_policy_opt} and Y~\cite{a,b,c}. We define safety as constraining the probability of a safety incident to be below some threshold, which corresponds to MDPs with constrained probability of constraint violation or CPMDPs~\cite{peter_geibel}."

% Second paragraph on methods: Prior methods have focused on a variety of challenges underlying safe RL, including off-policy learning and evaluation~\cite{stuff_eg_philip_thomas_work}, robustness to perturbations~\cite{robust_control,dro_for_rl,lerrel_pinto_robust_rl}, learning to reset to safe states~\cite{leave_no_trace}, and verifying the safety of a final policy~\cite{stuff_including_kochenderfer}. Like a number of prior works~\cite{stuff}, we focus on the problem of incorporating safety into the exploration and learning process. [summarize cvar,cpo,wcpg,other_non_learned methods; make it clear how our method differs from each class of methods, e.g. it scales to neural networks, it ensures safety during the learning process, it only requires sparse indications of safety incidents, etc]

\iffalse
\begin{figure}[t]
    \centering
    \vspace{0.2cm}
    \includegraphics[width=1.0\linewidth]{Figures/sqrl-diagram.pdf}
    \caption{\textbf{Illustration of our approach.} Our algorithm consists of two phases. In the first phase (left), our approach learns a safety-critic from experience. In the second phase (right), this learned safety-critic is used to constrain actions of new policies such that the process of learning something new is safe.}
    \label{fig:outline}
    %%BE.2.4: We should discuss whether we want to present the method as (1) a curriculum learning approach that ultimately results in safe learning; or (2) a safety masking idea. This figure conveys (1) but not (2). For (2), I think we'd want to highlight that the safety Q function can come from anywhere, and doesn't have to come from Q-learning/pre-training. I think the teaser figure we discussed before, which showed safe/unsafe actions in red/green did a better job of conveying (2).
    \vspace{-.1cm}
\end{figure}
\fi

% P1: Overview of definitions of safety, as defined by other RL papers
Our method builds on a rich body of work on safe RL~\cite{garcia2015comprehensive}. Prior works define safety in a variety of ways, using constraints on the expected return or cumulative costs~\cite{heger1994consideration, achiam2017constrained}, using risk measures such as Conditional Value at Risk and percentile estimates~\cite{Tamar2014PolicyGB,chow2014algorithms, duan2020distributional, ma2020distributional}, and defining regions of the state space that result in catastrophic or near-catastrophic failures \cite{lipton2016combating, eysenbach2017leave, fisac2019bridging}. We define safety as constraining the probability that a catastrophic failure will occur below a specified threshold, similar to how it is defined in prior work on MDPs with constrained probability of constraint violation (CPMDPs)~\cite{geibel2006reinforcement}.

% P2: Summarize some of the main methods/metrics used in previous papers that are most relevant
Researchers have determined a wide variety of challenges underlying safe RL, including lower-bounds on off-policy learning and evaluation~\cite{thomas2015high,dann2018policy}, robustness to perturbations~\cite{smirnova2019distributionally,pinto2017robust,xu2010distributionally}, learning to reset to safe states~\cite{moldovan2012safe, eysenbach2017leave}, and verifying the safety of a final policy~\cite{julian2019verifying}. One common focus of prior works is to learn a safe policy by minimizing worst-case discounted cost using conditional value at risk (CVaR) formulation~\cite{heger1994consideration,chow2017risk,tang2019worst}. However, these methods do not guarantee or offer ways to reason about the safety of policies attempted during the learning process. In contrast, we present a method of learning a safety layer that can adapt in parallel with a fine-tuned policy in an online fashion, making it better suited in the transfer learning setting where the environment or task has changed and the trained agent must safely adapt.
%Following prior work~\cite{dalal2018safe, Chow2019LyapunovbasedSP, achiam2017constrained, leike2017ai}, we focus on directly incorporating safety into exploration and learning. 

While there are many approaches to safety in RL, constrained MDPs are commonly used~\cite{altman1999constrained, achiam2017constrained, Tessler2018RewardCP}, where the agent optimizes the reward signal given constraints on the accumulated cost during the rollout. In work by \cite{chow2018lyapunov, Chow2019LyapunovbasedSP}, Lyapunov state-action functions are constructed using a feasible baseline policy, to enable safe Q-learning, policy gradient, and actor gradient methods, which map a learned policy into a space of policies that satisfy the Lyapunov safety condition. Similar to our work, this approach instills safety into the training process by directly evaluating every state's constraint cost. However, unlike these works, we do not assume well-defined, actionable safety criterion, and instead only access a sparse safety label which the agent uses to infer an actionable safety criterion and transfer it to new task instances.
%%CF.1.23: Can we put this in the long summary sentence, e.g. as "optimizing for a final policy that is safe~\cite{}"
%\cite{chow2017risk} proposes an algorithm which optimizes a policy with respect to the CVaR under selected risk constraints, by optimizing over the gradient of a corresponding unconstrained dual problem, but does not offer guarantees or ways to reason about the safety of policies attempted during the learning process.


%[summarize cvar,cpo,wcpg,other_non_learned methods; make it clear how our method differs from each
% Third paragraph on methods that learn notions of safety (e.g. prediction probability of collision, hans2008, learning to fly by crashing, etc.). Make it clear how our method generalizes some of the ideas in these prior works.

%%CF.1.23: Make sure to transition from the previous paragraph, and make it clear what these approaches are categorized (i.e. approaches to safety that incorporate learning into various aspects of the process.)
There have been many approaches to handling risk and safety in RL that have varied at an architectural level, which bear some similarities to our work. {In \cite{geibel2005risk}, Q-learning is adapted with an additional risk value estimate based on unsafe states to learn a deterministic policy that is risk-averse. } \cite{hans2008safe} proposed controlling a plant with RL, while learning a ``safety function'' from data to estimate a state's degree of safety, as well as a ``backup policy'' for returning the plant from a critical state to a safe regime. {However, neither approach tries transferring learned safety to a different task/environment with modified rewards or dynamics.}  \cite{eysenbach2017leave} showed a similar approach in a robotics domain, learning a ``reset policy'' to return a robot to its initial state distribution, which triggered if a corresponding value function drops below a certain threshold.
Our model builds on this idea by directly learning to predict failures, using this predictor to \emph{preemptively} filter unsafe actions, removing the need for an additional reset policy.
Additionally, we use our learned constraints to provide constrained updates to our policy during fine-tuning.

Finally, a number of works have learned models that predict the probability of future collisions for safe planning and control of mobile robots~\cite{richter2017safe,kahn2017uncertainty}. We instead aim to develop a general framework for many different modes of safety, and empirically observe the importance of several new design choices introduced in our algorithm on challenging continuous control problems.


%%CF.1.23: I would combine this with the above paragraph (for a single paragraph on approaches that use learning-based approaches to safety) and phrase this as: "Finally, a number of works have learned models that predict the probability of future collisions for safe planning and control of mobile robots~\cite{}. We instead aim to develop a general framework for many different modes of safety, and empirically observe the importance of several new design choices introduced in our algorithm on challenging continuous control problems."

%%CF.1.23: Can you make it clear what the benefits of our approach are here?

% Lastly, our work is developed using the maximum entropy reinforcement learning framework, which has had recent success in data-efficient methods capable of learning skills in robotic locomotion \cite{haarnoja2018learning} and in-hand manipulation environments \cite{haarnoja2018soft}. Additionally, our approach makes use of multiple Q-functions that are trained on different reward signals, making it comparable to methods that compose together multiple Q-functions to do policy optimization \cite{haarnoja2018composable}. However, one difference in our proposed approach is that we have designed one of the Q-functions to perform a safety evaluation on the current policy that is used to sample "safe" actions, making it capable of optimizing the policy for "safety tasks" concurrently with the selected evaluation task. Since we test our approach in multi-task applications, including learning a walking policy for the Minitaur, we use SAC as a baseline to compare against our approach.

==> Learning to be Safe - Arxiv/3-preliminaries.tex <==

% \subsection{Reinforcement Learning }

%%CF.1.20: This paragraph contains things that are specific to our problem setting, rather than just prior work needed to understand the method. This section should only contain old things. The safety things belong in the next section. You describe the MDP framework without describing how we modify it. We also don't actually modify the actual MDP framework itself. We just instantiate it with a particular terminal state corresponding to an unsafe event.

For our method, we consider the standard RL problem on a Markov Decision Process (MDP), which is specified by the tuple $\langle\mathcal{S}, \mathcal{A}, \gamma, r, P, \mu \rangle$. $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces respectively, $\gamma$ is a discounting factor, $r: \mathcal{S}\times \mathcal{A} \to \mathbb{R}$ is the reward function, and $P(\cdot|s,a)$ and $\mu$ are the state transition dynamics and initial state distributions respectively.
The aim of entropy-regularized reinforcement learning~\cite{ziebart2010modeling} is to learn a policy $\pi_\theta: \gS \times \gA \rightarrow [0, 1]$ that maximizes the following objective:
\begin{equation}
    J(\theta) = \sum_{t=0}^{T-1} \mathbb{E}_{(\mathbf{s}_t, \mathbf{a}_t) \sim \rho_\pi}[r(\mathbf{s}_t, \mathbf{a}_t) + \alpha \mathcal{H}(\pi_\theta(\cdot | \mathbf{s}_t))].
\end{equation}
We use $\gH(\pi_\theta(\cdot|s_t))$ to denote the policy's action entropy and $\alpha > 0$ as a tuning parameter.
% We choose use the soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft2}, noting that our approach can be combined with other off-policy RL algorithms.
%%BE.6.2: Cut above, as it's redundant w/ end of S5.1

\iffalse
    In the finite-horizon setting, the goal of the agent is to learn a policy $\pi_\theta: \mathcal{S}\times\mathcal{A}\to[0,1]$ that chooses which actions to take based on the current state in the environment. Given the reward function, the goal of the agent is to optimize the following objective: 
    \begin{equation*}
    J_\pi(\theta) = \sum_{t=0}^{T-1}\Big[\E_{(s_t,a_t)\sim\rho_\pi} \gamma^t r(s_t,a_t) \Big],
    \end{equation*}
    which corresponds to maximizing the total expected discounted return that results from following the policy $\pi_\theta$, where $\rho_\pi(s_t,a_t)$ refers to the state-action marginals induced by the policy $\pi$.
    
    % For our problem, we include a definition of the safety of a state-action pair as being encoded by a binary function $\mathcal{F}(s, a) $, where $\mathcal{F}(s, a) = 1$ if and only if action $a$ is \textit{unsafe}, and takes the agent to an unsafe state $s'$ that is terminal and indicates a catastrophic failure.
    
    To fully explore the space of safe behaviors, our approach leverages the framework of maximum entropy reinforcement learning~\cite{ziebart2010modeling} \st{that encourages exploration}, which uses the following RL objective: \vspace{-.15cm}
     % Mathematical presentation is confusing, e.g. line 148 expectation should be switched with the sum. Eq. (1) uses the probability of a failure state that should be just the indicator of the failure state.
    \begin{equation*}
    J_\pi(\theta) = \sum_{t=0}^{T-1} \mathbb{E}_{(\mathbf{s}_t, \mathbf{a}_t) \sim \rho_\pi}[r(\mathbf{s}_t, \mathbf{a}_t) + \alpha \mathcal{H}(\pi_\theta(\cdot | \mathbf{s}_t))].
    \end{equation*}
    Here, $\gH(\pi_\theta(\cdot|s_t)))$ is the entropy of the policy's distribution over actions at state $s_t$, and $\alpha$ is a weighting term. Although we choose use the soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft2}, for its sample efficiency, our approach is generally applicable, and can be combined with other off-policy RL algorithms. Next, we will formalize the problem setting that we consider.
\fi
    
%%%% EVERYTHING BELOW IS OLD/REWRITTEN

% In our setting, which involves pre-training and fine-tuning tasks, we assume that each task $\mathcal{T}_i$ is specified via its own MDP, either with changed rewards, dynamics, or initial state distributions. However, they all share a common task-agnostic safety-function, $\delta: \mathcal{S}\mapsto\{0,1\}$, which maps the state, irrespective of the task, to a safety label which says whether that state is terminal (due to a catastrophic/irrecoverable failure) or not. That is, $P(s|s,a) = 1$ for any action $a\in\mathcal{A}$ if $\delta(s) = 1$.

% Our reinforcement learning problem is to find an optimal policy in a modified Markov Decision Process (MDP) with certain \textit{unsafe} state-action pairs. The MDP has a state space $\mathcal{S}$, action space $\mathcal{A}$, and stochastic transition dynamics $p(s^\prime | s, a)$, which is the probability of arriving at state $s^\prime$ after taking action $a$ from state $s$. The distribution of initial states is $\mu(s)$. The agent receives a reward for taking action $a$ in state $s$, defined as $r(s,a)$. In our safety-aware MDP, there is a subset of states which terminate our finite-length episodes early, in some cases because of a catastrophic unsafe event. The safety of states is encoded with $\delta(s)\rightarrow \{0, 1\}$, where $\delta(s) = 1$ if and only if state $s$ is \textit{unsafe}.

%The safety of a state-action pair is encoded with a binary function $\mathcal{F}(s, a) $, where $\mathcal{F}(s, a) = 1$ if and only if action $a$ is \textit{safe} to take from state $s$, \textit{i.e.} taking action $a$ from state $s$ will not irrevocably take the agent to an unsafe state.

%%CF.1.20: I don't think the multi-task learning prelims really add anything, particularly since our problem setting is rather distinct. I commented it out.
%%CF.1.20: Also, I would recommend dropping the subsection dividers and having one merged section on RL notation and soft-actor critic.
\iffalse
\subsection{Multi-Task Learning}
To show how our framework can adapt and generalize, we show its performance in multi-task learning settings. Our tasks are drawn from a distribution $p(\mathcal{T})$, where each task $\mathcal{T}$ is an MDP which may have unique transition dynamics, reward function, and safety function. Each task in the distribution is at least analogous to all other tasks, with significant but reasonable differences, to make generalizing among tasks realistic.  We train our agents on a training distribution of tasks, then test on a new distribution of tasks to show how well our framework can acclimate and generalize to the new conditions, in both maximizing reward and maintaining safe patterns of behavior.
\fi


\iffalse
\subsection{Soft Actor-Critic Algorithm}

%%CF.1.20: I don't think the reader will understand why you're talking about multi-task learning and meta-learning. I also don't think this is the place to be motivating maxent RL. I would recommend saying something more like: "To explore the space of safe behaviors, our approach leverages the framework of maximum entropy reinforcement learning~\cite{ziebart}, which uses the following RL objective: $$<equation-here>$$. We will specifically use the soft actor-critic (SAC) algorithm~\cite{sac}, a sample-efficient off-policy method for MaxEnt RL. Though, our approach to safety is not specific to SAC, and only requires than an off-policy RL method be used. Next, we will formalize the problem setting that we consider."
%%CF.1.20: Even the above might be a bit more information than the reader really needs. But, it really depends on what information the methods section omits, and how it is written.
Within contexts of multi-task and meta-learning, an agent's robustness and ability to quickly generalize are especially important. A deterministic policy which performs well in a given task may be quite fragile and perform poorly in another task with seemingly minor differences. Intuitively, an agent which learns the most general policy possible to solve a given task, essentially learning as many different solutions as possible, will be better able to adapt to new tasks based on minor variations of the first task. This is the basic intuition behind maximum entropy RL methods~\cite{haarnoja2017reinforcement}. Maximizing entropy during learning prevents the agent from committing to a narrow hypothesis of the nature of the environment, instead keeping its hypothesis as broad as possible~\cite{ziebart2010modeling}.

While standard RL's objective is to maximize the sum over rewards, \cite{haarnoja2018soft} developed the SAC algorithm to maximize this objective augmented with the maximum entropy objective
\begin{equation}
    \label{eq:sac_cost} J(\pi) = \sum_{t=0}^T \mathbb{E}_{(\mathbf{s}_t, \mathbf{a}_t) \sim \rho_\pi}[r(\mathbf{s}_t, \mathbf{a}_t) + \alpha \mathcal{H}(\pi(\cdot | \mathbf{s}_t))]
\end{equation}
where $\rho_\pi((\mathbf{s}_t, \mathbf{a}_t)$ is the state-action marginal of the trajectory distribution induced by policy $\pi$, and $\mathcal{H}$ is the entropy.
\fi

==> Learning to be Safe - Arxiv/4-problem.tex <==
%%CF.1.20: Commenting out the subsection. Don't have a section with just a single section.
%\subsection{Task-Agnostic Safety}

%%CF.1.20: "our method" -- We're not talking about the method in this section! We're talking about the problem statement. I would also recommend starting with an informal description of the problem setting and then a more formal one. For example, you could start with something like: "Our goal is to enable an agent to learn how to be safe, and then use this learned notion of safety when learning new tasks. Our problem setting will hence be made up of two phases. The first phase is\emph{safety pre-training}, when ... The second phase ..."

In many robot learning settings, the conditions that lead to a catastrophic failure are difficult to fully specify before learning. While unsafe states are easily identifiable, such as the robot falling down or dropping an object, the task of formally specifying safety constraints that capture these states is non-trivial, and can be potentially biased or significantly hinder learning.

This is especially true if determining the agent's final behavior is difficult due to uncertainty about the underlying reward function and safety constraints. However, for many problems, the conditions for a catastrophic failure during an episode are easier to determine (e.g. determining that the robot has fallen down, or the object was dropped). Therefore, the challenge is to learn an optimal policy for a task while minimizing the frequency of catastrophic failures during training. To achieve this, we include 1) a safe pre-training environment, in which failures can be tolerated, and 2) a safety-incident indicator, $\mathcal{I}(s)$, which indicates if a given state is unsafe or not. In both the pre-training and target task environments, we treat these failure states as terminal. This setup enables the agent to learn to be safe and then transfer to new tasks without accumulating additional failure costs.

Under this framework, we propose learning in two phases: 1) learning an exploratory policy that solves a simpler/safer task in the pre-training environment, and 
2) \textcolor{black}{transferring the learned policy to} a more safety-critical target task with guarantees to safety. Our \emph{safety-aware} MDP for the pre-training and target tasks are respectively defined as $\mathcal{T_\text{pre}} = \langle \mathcal{S}, \mathcal{A}, P_\text{pre}, r_\text{pre}, \mu_\text{pre}, \mathcal{I} \rangle$, and $\mathcal{T_\text{target}} = \langle \mathcal{S}, \mathcal{A}, P_\text{target}, r_\text{target},\mu_\text{target},  \mathcal{I} \rangle$. 
% Formally,
% our reinforcement learning problem becomes finding an optimal policy where,
After pre-training in a safety test-bed task ($\ptask$), the agent must optimize its expected return in the target training task ($\gtask$) while minimizing visits to unsafe states:
% how frequently it reaches unsafe states. This makes the goal of policy learning %\vspace{-.3cm}
\begin{align*}
\max_{\pi} \sum_{t=0}^T \E_{(s_t,a_t)\sim \rho_\pi}
\left[r_\text{target}(s_t, a_t) \right] ~ \textrm{s.t.}\; \E_{s_t \sim{\rho_\pi}}\left[\mathcal{I}(s_t)\right] < \esafe. \;
% \label{eq:target-obj}
\end{align*}
This objective implies that for the target task, the policy should always stay outside of the unsafe region $\sunsafe = \{s \;|\; \gI(s) = 1\}$ with probability $\esafe$.
This also introduces the notion of a target safety threshold, $\esafe$, which serves as an upper-bound on the expected risk \textcolor{black}{of a given policy}. When used as a single-step constraint over actions sampled during policy rollouts, it can guarantee that the policy $\pi$ is safe up to that threshold probability under certain assumptions. Importantly, we aim to impose this safety constraint not just at convergence, but throughout the training process. %In our practical algorithm, we solve this CMDP using the Lagrangian method, with a constraint on penalty violation~\cite{altman1999constrained}.
%%CF: I'm commenting out this last sentence because it seems more about the method than the problem.


==> Learning to be Safe - Arxiv/5-method.tex <==
%%CF.1.20:  This methods section is a bit scattered, making it hard to follow and understand the method. Further, it is very terse -- you should expect it to be a page or more. Be sure to describe everything in the text rather than relying on the algorithm to convey the method.
%%CF.1.20: To make it less scattered, I would recommend a top-down organization as follows:
%% *Intro paragraph* on what happens in the two phases -- use the terms that you introduced in the problem statement section, convey the intuition of the method. Leave out implementation details.
%% *Subsection* on what happens during pretraining: 
% Start by describing the goal, i.e. learning a Q-function that predicts the safety of actions under downstream policies. Then, define what a safety Q-function is, i.e. "Q_safe^pi corresponds to the probability that ...." Key questions then lie in (a) how do we train such a function, (b) with what data do we train it, and (c) for what policy pi?
% Then say that there's a reason why we've been calling it a safety \emph{Q-function}. We can train it using dynamic programming! Write down the corresponding Bellman equation. This answers (a).
% For (b), we want to train it on diverse data to seek out unsafe states, and particularly unsafe states that are nearby the kinds of tasks we might be asked to perform in the future. Hence, we will use maximum entropy RL with the rewards available in the safety pre-training phase. 
% This leaves (c), which is a very important challenge.The safety model may be overly pessimistic if trained on data from very diverse, random policies. To address this challenge, we will learn to model safety only for the set of policies that are constrained by the safety model itself, using a simple modification to the objective. Use this to write out the final objective. 
% Finally, refer readers to an algorithm box that only describes the pre-training phase, not the training phase.
%% *Subsection* on what happens during training
% Brief motivation on how we want to be safe during the learning process.
% Describe how the policy used to collect data is constrained by the Q_safe from the pre-training phase. Write down an equation to make it clear how it is constrained. Also, make it clear if the policy update changes (I can't remember if it does or not)
% Then, motivate and then describe how you also fine-tune the safety-critic during this phase, as needed.
% Refer to separate algorithm box for what happens during the main training phase.

%% After, this section should be a *separate* section on implementation details that include things (i) we choose to use SAC, (ii) how things connect to SAC, (iii) things like CEM

%%CF.1.20: Lastly, as you write the section, make sure to *briefly* motivate each of your algorithm decisions.

%%CF.1.26: This paragraph should only contain English and a few symbols. Leave equations for the corresponding subsections. Here's one way it can be written: "To address the problem statement described above, we will aim to simultaneously learn a policy and a notion of safety in the first phase, and then fine-tune this policy for the target task using the learned safety precautions. As a result, we can ensure safety in the second phase during the learning process itself. To do so, we will learn a safety Q-function, $\qsafe^\pi$, that predicts the safety of future behavior starting from a given state, action pair, and then use $\qsafe^\pi$ to constrain the actions taken during fine-tuning.  In this section, we will describe our approach, safety Q-functions for reinforcement learning (SQRL) and analyze it's performance."

To address the problem formulation described above, we introduce the Safety Q-functions for Reinforcement Learning (SQRL), which simultaneously learns a policy and notion of safety in the first phase, and later fine-tunes the policy to the target task using the learned safety precautions. In turn, the safety in the second phase of training can be ensured during the learning process itself. This is done by the safety-critic, $\qsafe^{\bar{\pi}}$, which estimates future failure probability of a safety-constrained policy given a state, action pair. The safety-constraints learned by $\qsafe^{\bar{\pi}}$ can induce the policy to be safe, even when the task has changed. In this section, we will describe our approach and analyze its performance.

\subsection{Pre-Training Phase}

%%CF.1.26: See my notes above for what should go in this section (which I also copied below). you need to formally describe how pre-training is done -- define what the safety Q function represents, including the discount factor. 
%% Describe how the discount factor can be interpreted. 
%% Write down the "Bellman" equation for the safety-Q function. 
%% Then motivate and write down the equation for the version where the policy is constrained by the safety Q function itself. Everything needs to be formally written out in equations.
During pre-training, the goal is to learn a safety-critic $\qsafe^{\bar{\pi}}$ and the optimal pre-trained policy $\pi_\text{pre}^*$ which will serve as the initialization for training on the target task.  For our problem, the optimal safety-critic for the pre-training task $\ptask$ estimates the following expectation for a given policy $\pi$:
% Reviewer comment: Further, the optimal Q*_safe does not correspond to the Q^pi_safe on line 215 that introduces a discount factor and no more represents a probability of a failure.
\begin{equation}
Q_\text{safe}^{\pi}(s_t, a_t) = \gI(s_t) + (1-\gI(s_t))
    %\E_{\substack{s_{t'} \sim P_\text{pre}(\cdot|s_t, a_t) \\ a_{t'} \sim \pi(\cdot|s_{t'})}}  \qsafe^\pi (s_{t'}, a_{t'}) 
    %\E_{\substack{s_{t'} \sim P_\text{pre}(s_{t'-1}, \pi(s_{t'-1}))}} \left[ \gsafe^{t'-t} \mathcal{I} (s_{t'})\right],
    \sum_{t'=t+1}^T
    \E_{\substack{ s_{t'} \sim P_\text{pre}(\cdot | s_t, a_t) \text{ for } t'=t+1\\
    s_{t'} \sim P_\text{pre}, \pi \text{ for } t'>t+1
    }} \left[
    \gsafe^{t'-t} \mathcal{I} (s_{t'})
    \right],
\label{eq:failure-prob}
\end{equation}
The target failure estimate $Q_\text{safe}^\pi$ estimates the true probability that {$\pi$} will fail in the future if, starting at state $s_t$, it takes the action $a_t$. This raises two key questions: 1) how should such a model of safety be trained, 2) with what data do we train it, and 3) for what policy $\pi$ do we train it?

%% TODO: Add ablation showing that training safety-critic with Bellman equation for failure instead of normal supervised learning yields better safe-policy performance (just show for the 2D maze environment)

Regarding the first question, if the safety-critic were a binary classifier, supervised learning could be used to just estimate the safety labels for a single timestep. However, to learn the cumulative failure probability in the future, the safety-critic must reason over future timesteps also. Hence, the safety-critic is trained using dynamic programming, as in standard Q-learning, using a discount term, $\gsafe$, to limit how far in the past the failure signal is propagated. This cumulative discounted probability of failure is estimated by the Bellman equation:% corresponding to the probability of safety as:
\begin{equation*}
\hat{Q}_\text{safe}^{\pi} (s, a) = \gI(s) + (1 - \gI(s))
    \mathbb{E}_{\substack{s' \sim P_\text{pre}(\cdot|s,a)\\ a'\sim \pi(\cdot|s')}}
        \left[ \gsafe \hat{Q}_\text{safe}^{\pi}(s', a')\right].
\end{equation*}
Parametrizing the safety Q-function $\hat{Q}_\text{safe}^\pi$ as a neural network with parameters $\psi$ yields the following objective:
\begin{align}
    J_{\text{safe}}(\psi) = \E_{(s ,a, s', a')\sim \rho_\pi} \bigg[\bigg( \hat{Q}_\text{safe}^\pi(s,a) - \nonumber 
    \left(\gI(s) + (1 - \gI(s)) \gsafe \bar{Q}_\text{safe}^\pi(s', a')\right) \bigg)^2 \bigg],
    %\tilde{Q}^\text{safe} (s',a') \right)^2 \right],
\end{align}
where $\bar{Q}_\text{safe}$ corresponds to the delayed target network.

\begin{figure*}[ttt!]

\begin{minipage}[t]{2.76in}
\begin{algorithm}[H]
\caption{SQRL Pre-training}\label{alg:sqrl-pre}
\begin{algorithmic}[1]
\Procedure{Pretrain}{$n_\text{pre}, \ptask, \esafe, \gsafe$} \label{safesac-pretrain}
\State Initialize replay buffers, $\gD_\text{safe}, \gD_\text{offline}$
\State Initialize networks, $\hat{Q}_\text{safe}^\psi, \pi_\theta, Q_{\phi_1}, Q_{\phi_2}$.
\State $s \sim \mu_\text{pre}(\cdot)$
\For{$n_\text{pre}$ steps} %\Comment{Begin pre-training phase}
\For{$n_\text{off}$ steps} %\Comment{train off-policy method}
    \State Sample action, $a \sim \pi_\theta(\cdot | s)$
    \State $s' \sim P_\text{pre}(\cdot|s,a)$
    \State $\gD_\text{offline}\text{.add}((s, s', a, r_\text{pre}(s, a)))$
    % \State $\theta, \phi_1, \phi_2 \gets$ \Call{SACUpdate}{$\theta, \phi_1, \phi_2, \gD_\text{offline}$}
    % \LeftComment{Perform SAC update on actor, critic, $\alpha$}
    \State Apply SAC update to $\theta$, $\phi_1$, $\phi_2$, $\alpha$
    % \State $\theta \gets \theta - \lambda_\theta \hat{\nabla}_\pi J_\pi(\theta,\alpha)$
    % \State $\phi_i \gets \phi_i - \lambda_{\phi_i} \hat{\nabla}_{\phi_{i}} J_Q(\phi_i)$ for $i\in\{1,2\}$
    % \State $\alpha \gets \alpha - \lambda_{\alpha} \hat{\nabla}_\alpha J(\alpha)$
    \If {$\gI(s') = 1$} $s' \sim \mu_\text{pre}(\cdot)$\EndIf
    \State $s \gets s'$
\EndFor
\LeftComment{{\fontfamily{cmtt}\selectfont \textcolor{blue}{// Collect $k$ on-policy rollouts}}}
\For{$i \gets 1,k$ episodes}
    \State $\tau_i \gets$ \Call{Rollout}{$\bar{\pi}_\theta, \ptask$}
    \State $\gD_\text{safe}\text{.add}(\tau_i)$ 
\EndFor
\State $\psi \gets \psi - \hat{\nabla}_\psi J_\text{safe}(\psi)$
\EndFor
\Return{$\pi_\theta, \hat{Q}_\text{safe}^\psi$} \label{safesac-pretrain-end}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{2.76in}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\caption{SQRL Fine-tuning}\label{alg:sqrl-fine}
\Procedure{Finetune}{$n_\text{target}, \gtask$, $\hat{Q}_\text{safe}$} \label{safesac-finetune}
\State  $s \sim \mu_\text{target}(\cdot)$, $\;\gD_\text{offline} \gets \{\}$
\For{$n_\text{target}$ steps}
    \State Sample action, $a \sim \bar{\pi}_\theta(\cdot |s)$
    \LeftComment{{\fontfamily{cmtt}\selectfont \textcolor{blue}{// where $\bar{\pi}_\theta~\gets~\Gamma(\pi_\theta)$ (Eq.~\ref{eq:safe-pi})}}}
    \State $s'~\sim~P_\text{target}(\cdot|s,a)$
    \State $\gD_\text{offline}\text{.add}((s, s', a, r_\text{target}(s, a)))$
    \LeftComment{{\fontfamily{cmtt}\selectfont \textcolor{blue}{// Dual gradient ascent on Eq.~\ref{eq:pol-ft}}}}
    \State{ $\theta~\gets~\theta~+~\lambda \hat{\nabla}_\theta J_{\text{target}}(\theta,\alpha,\nu)$}
    % \State{ $\alpha, \nu \gets \theta + \lambda \hat{\nabla}_\theta J_{\text{target}}(\theta, \alpha, \nu)$}
    \State $\alpha~\gets~\alpha~-~\lambda \hat{\nabla}_\alpha J_\text{target}(\theta,\alpha,\nu)$
    \State $\nu~\gets~\nu~-~\lambda \hat{\nabla}_\nu J_\text{target}(\theta,\alpha,\nu)$
    
    \If{$\gI(s') = 1$} $s' \sim \mu_\text{target}(\cdot)$\EndIf
    \State $s \gets s'$
\EndFor
\Return{$\pi_\theta$} \label{safesac-finetune-end}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-5mm}
\end{figure*}


For the safety model to learn new tasks without failure, it must first explore a diverse set of state-action pairs, including unsafe state-action pairs, during pre-training. This motivates using maximum entropy reinforcement learning, which encourages exploration by maximizing both the reward and the entropy of the policy. In our implementation, we choose the soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft}, though in principle, any off-policy algorithm can be used as long as it explores sufficiently. 

Finally, we must determine which policy to optimize the safety-critic under. If we use the entirety of training experience from SAC, which contains data from a mixture of all policies encountered, this may result in a safety Q-function that is too pessimistic. For example, if the mixture of policies includes a random, unsafe policy from the start of training, then even a cautious action in one state may be considered unsafe, because risky actions are observed afterwards. Therefore, we are faced with a dilemma: while we need diverse data that includes a range of unsafe conditions, we also need the actions taken to be reflective of those taken by safer downstream policies constrained by the safety-critic to avoid learning a pessimistic safety-critic. To address this conundrum, the safety-critic is optimized under the mixture of policies that are constrained by the safety-critic itself which we denote as $\bar{\pi}_i$ where $i$ is the iteration. This mitigates pessimism, since for a safe state-action pair in the data, subsequent behavior from that point will be constrained as safe, hence producing a reliable target label. %To achieve this, we deliberately bias our samples from $\pi(a \mid s)$ during training to have failure probability near the target threshold, $\esafe$, so that they can teach the safety-critic which actions actually cause failures and which ones are safe.
%%CF: This above sentence is already mentioned in the practical implementation, so I think it's okay to omit here.

%However, training a standard MaxEnt RL policy during this phase may lead the safety-critic to becoming overly pessimistic, since the data collected during this phase will be from policies that are trying to optimize diversity of sampled actions.

% This process deliberately biases the action sampling to get better at sampling actions that are near the threshold, is that necessarily good? 

To this end, the safety-critic and a stochastic safety-constrained policy $\bar{\pi}_\epsilon(a \mid s)$ are jointly optimized during pre-training.
%During pre-training, the goal is to train a safety-critic that can accurately predict the failure probability (Eq.~\ref{eq:failure-prob}), and be used to reject samples $a \sim \pi(a \mid s)$ when they have a high probability of failure, $\qsafe^\pi(s,a) > \esafe$. 
Let the safety policy $\bar{\pi}_\epsilon$ be a policy that has zero probability of sampliing an action $a$ where $\hat{Q}_\text{safe}(s,a) \geq \epsilon$. Let the set of all policies where this holds be $\Pi_\text{safe}^\epsilon$. Next, the projection $\Gamma^\epsilon_\text{safe} : \pi \rightarrow \bar{\pi}_\epsilon \in \Pi^\epsilon_\text{safe}$ be the projection mapping any policy onto its closest policy in $\Pi_\text{safe}$. Consi a natural projection operator, using our safety-critic definition, that does the following:
\vspace{-.1cm}
\begin{equation}
    \bar{\pi}(a \mid s) \propto \begin{cases} \pi(a \mid s) & \text{if } \hat{Q}_\text{safe}^\pi(s, a) \le \epsilon \\ 0 & \text{otherwise} \end{cases}.
    \label{eq:safe-pi}
\end{equation}
By masking the output distribution over actions from $\pi$ to only sampling actions where this safety condition is met, the policy $\bar{\pi}$ is ensured to be safe.
% This definition now allows us to outline the final procedure of our pre-training process.

Our pre-training process, summarized in Algorithm~\ref{alg:sqrl-pre}, proceeds as follows.
Let $\epsilon=\esafe$ define our target safety threshold, beyond which actions should be rejected for being too risky. Then, at each iteration of training, we collect data from our current policy with actions constrained by the current safety-critic (i.e. projecting our policy into $\Pi_\text{safe}^{\epsilon}$), add the data to our replay buffer, update our safety-critic under the mixture of policies represented in the replay buffer, and update our policy using a MaxEnt RL algorithm.
% The result of this pre-training is a safe policy that solves the pre-training task, $\bar{\pi}_\text{pre}$ and a safety Q-function $\qsafe^\pi$. 
Pre-training returns a safe policy that solves the pre-training task, $\bar{\pi}_\text{pre}$, and a safety Q-function $\hat{Q}_\text{safe}$. 
% The full pre-training process is outlined in Algorithm~\ref{alg:sqrl-pre}.

% \todo{need to formally describe how this is done, using equations. I think we should put the projection operator here, since it is needed to understand how pre-training is done.}
% \todo{the stuff below on how to sample actions belongs in a separate section on implementation. I copied it there}

\vspace{-0.1em}
\subsection{Fine-Tuning Phase}
\vspace{-0.1em}
In the fine-tuning phase, SQRL initializes the policy to the safety-constrained pre-training policy $\bar{\pi}_\text{pre}$ and fine-tunes to a new safety-critical target task $\mathcal{T_\text{target}}$. To do this, we formulate a safety-constrained MDP using the pre-trained safety-critic $\hat{Q}_\text{safe}$. While fine-tuning on the target task, all data is collected using policies that are constrained by $\hat{Q}_\text{safe}$, following the data collection approach used in pre-training, and the policy is updated with respect to the target task reward function. We additionally add a safety constraint cost to the policy objective to encourage the unconstrained policy $\pi'$ to sample actions that will fall within the distribution of $\Gamma^\epsilon_\text{safe}(\pi') = \bar{\pi}'_\epsilon$, while optimizing for expected return. This modifies the standard soft-actor policy objective to 
\begin{align*}
    J_\text{target}(\theta, \alpha, \nu) = \E_{\substack{(s, a) \sim \rho_{\bar{\pi}_\theta'}\\ a' \sim \pi'_\theta(\cdot | s)}} \Big[ 
    r_\text{target}(s, a) - \alpha(\log\pi_\theta'(\cdot | s) - \bar{\mathcal{H}}) + \nu\big(\esafe - \hat{Q}_\text{safe}(s, a')\big)\Big], \numberthis
    \label{eq:pol-ft}
\end{align*}
where $\alpha$ and $\nu$ are Lagrange multipliers for the entropy and safety constraints respectively, and where $\bar{\mathcal{H}}$ denotes the target entropy (a hyperparameter of SAC). Algorithm~\ref{alg:sqrl-fine} summarizes the fine-tuning process.



\vspace{-0.1em}
\subsection{Analysis}
\vspace{-0.1em}

Next, we theoretically analyze the safety of SQRL, specifically considering the safety of the learning process itself. 
For this analysis (but \emph{not} in our experiments), we make the following assumptions:
\begin{assumption}
The safety-critic $\hat{Q}_\text{safe}^{\bar{\pi}}$ is optimal such that, after pre-training, can estimate the true expected future failure probability given by ${Q}_\text{safe}^{\bar{\pi}}$ in Equation~\ref{eq:failure-prob}, for any experienced state-action pair.
\label{assump1-s5}
\end{assumption}
\begin{assumption}
The transition dynamics leading into failure states have a transition probability at least $\epsilon$. That is, for all unsafe states $s' \in \gS_\text{unsafe}$, $P(s'|s, a) > \epsilon$ or $P(s'|s, a)=0$  $\forall (s, a)$.
\label{assump2-s5}
\end{assumption}
\begin{assumption}
The support of the pre-training data for $\qsafe^\pi$ covers the states and actions observed during fine-tuning.
\label{assump3-s5}
\end{assumption}
\begin{assumption}
There always exists a ``safe'' action $a$ at every safe state $s \not\in \gS_\text{unsafe}$ that leads to another safe state (i.e. $\exists a, s' : \gI(s') = 0 \; \text{s.t.} \; P(s' | s,a) > 0$ if $\gI(s) = 0$).
\label{assump4-s5}
\end{assumption}

\begin{lemma}
For any policy $\bar{\pi} \in \Pi_\text{safe}^\epsilon$, the discounted probability of it failing in the future, given by $\E_{s_{t'} \sim \rho_{\bar{\pi}}|s_t}(\gsafe^t \gI(s_{t'}) \mid t' > t)$, is less than or equal to $\esafe$, given a safety-critic $\qsafe^{\bar{\pi}}$.
\label{lem:1}
\end{lemma}

% Add proof to the Lemma 1
Assuming that $\hat{Q}_\text{safe}^{\bar{\pi}} = Q_\text{safe}^{\bar{\pi}}$ (Assumption 1), for the base case we can assume for a policy $\bar{\pi}$ starting in state $s_0 \in \mathcal{S}_\text{safe},$ there is always an action $a_0$ for which $\pi(a_0|s_0) > 0$ and $\hat{Q}_\text{safe}(s_0,a_0) < \esafe$:
% then following from the definition of $\bar{\pi}$ and $Q_\text{safe}^*$.:
% \vspace{-.15cm}
\begin{equation*}
    \hat{Q}_\text{safe}^\pi(s_0, a_0) = \E_{\bar{\pi}}
    \left[\gsafe^t \mathcal{I}(s_t) | t \geq 0\right] = \Pr(\mathcal{I}(s_0) = 1) + \E_{\pi}\left[\gsafe^t \mathcal{I}(s_t) | t > 0\right] < \esafe.
    % \vspace{-.25cm}
\end{equation*}
From recursion, it follows that when the step probability of failing is below $\esafe,$ if the policy $\bar{\pi}$ masks the actions sampled by $\pi$ to those that are within the safety threshold, $\hat{Q}_\text{safe}^{\bar{\pi}}(s_t, a_t) < \esafe$, $a_t \sim \bar{\pi}_\epsilon(s_t)$ has failure probability less than $\hat{Q}_\text{safe}^{\bar{\pi}}(s, a).$  This is because there are actions in the support of the expectation of $\hat{Q}_\text{safe}^{\bar{\pi}}(s, a)$ where $\Pr(\mathcal{I}(s_t) = 1) < \esafe,$ or else that state's cumulative failure probability would be $> \epsilon.$ From Assumptions 2 and 3, this means that these actions can be sampled by $\bar{\pi}$, and from the definition of the masking operator $\Gamma_\text{safe}^\epsilon$, actions that would violate the constraint are masked out. A visual representation of this concept is presented in Fig.~\ref{fig:safety_mask} in Appendix~\ref{appendix:A}.
% Lemma 1, say something stronger, that all of the policies trained will be safe
\begin{theorem}
Optimizing the policy learning objective in Eq.~\ref{eq:pol-ft}, given from Assumptions 1-4, all new policies $\pi'$ encountered during training will be in $\Pi_\text{safe}^\epsilon$ when trained on $\gtask$.
\label{thm:1}
\end{theorem}
Following from Lemma~\ref{lem:1}, we can show that actions sampled according to the projected safety policy $\bar{\pi}'$ match the constraints that $Q_\text{safe}^* < \esafe$ and therefore makes the problem equivalent to solving the CMDP $(\mathcal{S}, \mathcal{A}, P_\text{target}, \mu, r_\text{target}, \qsafe)$, where the constraints are learned in the pre-training phase. A more detailed proof is included in the supplemental material.


\section{Practical Implementation of SQRL}

To train a safety-critic and policy with SQRL on high-dimensional control problems, we need to make several approximations in our implementation of the algorithm which in practice do not harm overall performance. Our method is implemented as a layer above existing off-policy algorithms which collect and store data in a replay buffer that is used throughout training for performing updates. For our method, we store trajectories in an offline replay buffer, $\gD_\text{offline},$ when collecting samples for training the actor and critic, and additionally keep a smaller, ``on-policy'' replay buffer $\gD_\text{safe}$, which is used to store $k$ trajectories samples from the latest policy to train the safety-critic, after training the policy offline for $n_\text{off}$ steps. During pre-training, we use rejection sampling to find actions with a failure probability that are only just below the threshold $\esafe$, scored using the current safety-critic.
%safe actions with a failure probability below the threshold $\esafe$ are rejection-sampled, scored using the current safety-critic. 
This equates to sampling safe but `risky' actions that encourage the agent to explore the safety boundary to correctly identify between safe and unsafe actions for a given state. Alternatively, methods like cross entropy method which perform importance-based sampling weighted by the safety-critic failure probability could also be used.

Sampling actions in this way affects the algorithm by ensuring the data being collected by our method during policy evaluation gives the safety-critic the most information about how well it determines safe and unsafe actions close to the threshold of $\esafe$. Since the behavior of the final safety policy is largely determined by the safety hyperparameters $\esafe$ and $\gsafe$, which are task and environment-specific, one additional step during pre-training is tuning both of these parameters to reach optimal pre-training performance, since it is unsafe to tune them while attempting to solve the target task.

In the fine-tuning phase, the safe sampling strategy translates into selecting safe actions according to $\qsafe^{\bar{\pi}}$ by, once again, sampling $k$ actions, masking out those that are unsafe, and then importance sampling the remaining options with probability proportional to their log probability under the original distribution output by $\pi(\cdot |s)$. In the event that no safe action is found, the safest action with lowest probability of failing is chosen. Qualitatively in our experiments, these are typically actions that stabilize the robot to avoid failure, and restrict the ability to accumulate reward for the remainder of the episode.
In our experiments in Section~\ref{sec:experiments}, we show ablation results that confirm the benefit of the exploration induced by MaxEnt RL to improve the quality of safety exploration during pre-training, yielding a better quality estimate of failure probabilities when the goal task is attempted.

\iffalse
First, we define a safety policy $\bar{\pi}_\epsilon$ as a policy whose actions where $\qsafe(s,a) \geq \epsilon$ have probability 0. Let the set of all policies where this holds be $\Pi_\text{safe}^\epsilon$. Next, we define the projection $\Gamma^\epsilon_\text{safe} : \pi \rightarrow \bar{\pi}_\epsilon, \bar{\pi}_\epsilon \in \Pi_\text{safe}$ that maps any policy onto this set. Let us consider a natural projection operator, using our safety-critic definition, that does the following: 
\vspace{-.1cm}
\begin{equation}
    \bar{\pi}(a \mid s) \propto \begin{cases} \pi(a \mid s) & \text{if } Q_\text{safe}(s, a) \le \epsilon \\ 0 & \text{otherwise} \end{cases}.
    \vspace{-.1cm}
\end{equation}
By masking the output distribution over actions from $\pi$ to only sampling actions where this safety condition is met, the policy $\bar{\pi}$ is ensured to be safe, where $\qsafe^\pi$ plays a similar role as the safety-layer used in~\cite{dalal2018safe}. 
\fi

==> Learning to be Safe - Arxiv/6-experiments.tex <==

In our experimental evaluation, we aim to answer the following questions {to evaluate how well our method transfers in this task-agnostic setting}: (1) Does our approach enable substantially safer transfer learning compared to RL without a safety-critic? (2) How does our approach compare to prior safe RL methods? (3) How does SQRL affect the performance, stability, and speed of learning? (4) Does tuning the safety threshold $\esafe$ allow the user to trade-off risk and performance?

\textbf{Environments.} 
% TODO: ADD % of total reward side by side with failure rate
\begin{figure*}
  \begin{minipage}{.565\textwidth}
  \centering
  \begin{subfigure}[b]{.99\linewidth}
  \centering
      \includegraphics[width=0.99\linewidth]{Figures/bar-plots.pdf}
      \label{fig:bar-plot}
      \vspace{-0.5cm}
  \end{subfigure}
  \caption{\small Final task performance and cumulative failure rate during fine-tuning. SQRL achieves good performance while also being significantly safer during learning. }
  \end{minipage}% \hfill
  \hfill
  \begin{minipage}{.42\textwidth}%[t][][b]{.65\textwidth}
  \begin{subfigure}[b]{.99\linewidth}
    \includegraphics[width=1.0\linewidth]{Figures/sqrl_envs.png}
    \vspace{-0.5cm}
  \end{subfigure}
  \caption{\small Environments used in the paper}
    % \begin{subfigure}[b]{.95\linewidth}
    %     \centering
    %     \includegraphics[height=2cm]{Figures/minitaur-1.png}
    %     \caption{\small Minitaur}
    %     \label{fig:mini-env}
    % \end{subfigure}
    % \begin{subfigure}[b]{.45\linewidth}
    %     \centering
    %     \includegraphics[height=2cm]{Figures/envs.pdf}
    %     \caption{\small Cube Rotation}
    %     \label{fig:cube-env}
    % \end{subfigure}
    % \centering
    % \begin{subfigure}[b]{.45\linewidth}
    %     \centering
    %     \includegraphics[height=2cm]{Figures/drunkspider.png}
    %     \caption{\small Drunk Spider}
    %     \label{fig:drunk-env}
    % \end{subfigure}
    % \vspace{-1em}
    %\vspace{-0.3cm}
    \label{fig:envs}
  \end{minipage} %\quad
\end{figure*}
To answer these questions, we design our experiments in three distinct environments, shown in Figure~\ref{fig:envs}. Inspired by~\citet{kappen2005path}, the \textbf{drunk spider} domain is a 2D navigation environment, where the agent must learn to navigate to a fixed goal position, with stochastic dynamics corresponding to action noise. There is a narrow bridge that goes directly from start to goal, with two lava pits on either side. Falling into either pit corresponds to a failure and episode termination. If the agent is unconfident about crossing the bridge without falling, it can instead choose to go around the bridge and lava pits entirely, which takes longer (\textit{i.e.}, costs more) but avoids the risk of falling. Our second environment is the \textbf{minitaur} quadruped locomotion environment from~\citet{tan2018sim}. Here, we consider the task of running at faster speeds, i.e. 0.4 m/s, after pre-training on a safer desired velocity of 0.3 m/s, with the goal of learning to run without falling. We also include a variant of this environment that increases the foot friction of the simulator during fine-tuning, showing that our method works even when there are changes in the environment dynamics.
Our last environment corresponds to \textbf{cube rotation} with a five-fingered 24 DoF ShadowHand using the environment introduced by~\citet{nagabandi2019deep}. The goal is to rotate a cube from a random initial orientation to a desired goal orientation, where the fine-tuning task requires a larger orientation change than the pre-training phase. An unsafe state corresponds to the block falling off the hand.
See Appendix~\ref{appendix:env} for details.

\subsection{The Performance and Safety of Learning}

To answer question (1), we perform an ablation of our approach where no safety-critic training is performed. This comparison directly corresponds to training standard SAC on the pre-training task, and fine-tuning the pre-trained policy on the target task, {shown in Figure~\ref{fig:safety_stability}}.
This directly compares the role the safety-critic plays in both safety and performance. To address question (2), we compare SQRL to four prior approaches for safe reinforcement learning: worst cases policy gradients (WCPG)~\cite{tang2019worst}, which learns a distribution over Q-values and optimizes predicted worst case performance, ensemble SAC (ESAC), which uses an ensemble of critics to produce a conservative, risk-averse estimate of the Q-value during learning~\cite{eysenbach2017leave}, constrained policy optimization (CPO), which adds a constraint-based penalty to the policy objective~\cite{achiam2017constrained}, and Risk-Sensitive Q-Learning (RS), which adds the risk estimate directly to the reward objective~\cite{geibel2005risk}. To compare to~\cite{geibel2005risk}, we re-use the pre-trained SQRL policy and penalize the critic loss with the safety-critic risk estimate scaled by a Lagrange multiplier. For all prior methods, we perform the same pre-training and fine-tuning procedure as our method to provide a fair comparison.

We compare all of the methods in fine-tuning performance in Figure~\ref{fig:safety_stability}. Overall, we observe that SQRL is substantially safer, with fewer safety constraint violations, than both SAC and WCPG, while transferring with better final performance in the target task. In the drunk spider environment, all approaches can acquire a high performing policy; however, only SQRL enables safety during the learning process, with only a 1\% fall rate.
In the Minitaur environment, SQRL enables the robot to walk at a faster speed, while falling around only 5\% of the time during learning, while the unconstrained SAC policy fell about 3x as often. Finally, on the challenging cube rotation task, SQRL achieves good performance while dropping the cube the least of all approaches, although SAC performs better with more safety incidents.


%In particular, on the Minitaur locomotion task, our method succeeds at enabling the robot to walk at a faster speed without falling as often as SAC or WCPG.


% \todo{describe results here, referring to bar plots}


\begin{figure*}
\centering
    %\begin{subfigure}[b]{.32\linewidth}
      %  \includegraphics[width=0.32\linewidth]{Figures/minivel-finetune.png}
        % \caption{Total failure rate during fine-tuning}
       % \label{fig:min-vel-ret-ft}
    %\end{subfigure}
    %\begin{subfigure}[b]{.32\linewidth}
      %  \includegraphics[width=0.32\linewidth]{Figures/minifric-finetune.png}
        % \caption{Total failure rate during fine-tuning}
     %   \label{fig:min-vel-ret-ft}
    %\end{subfigure}
    %\begin{subfigure}[b]{.32\linewidth}
       % \includegraphics[width=0.32\linewidth]{Figures/cuberotate-finetune.png}
        % \caption{Total failure rate during fine-tuning}
      %  \label{fig:min-vel-ret-ft}
    %\end{subfigure}
    \includegraphics[width=0.99\linewidth]{Figures/finetune_combined_biglegend.png}
    \vspace{-0.1cm}
    \caption{Fine-tuning curves for our method on the Minitaur and Cube target tasks, suggesting that, beyond increasing safety, SQRL's safety-critic leads to more stable and efficient learning.}
    \label{fig:safety_stability}
    \vspace{-1em}
\end{figure*}

\subsection{The Effect of Safety on Learning}

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-2em}
    \centering
    \includegraphics[width=1\linewidth]{Figures/safe-vs-risky_cropped.pdf}
    \vspace{-0.2cm}
    \caption{\small Qualitative results showing different trajectories corresponding to different target safety thresholds.}% By tuning the safety threshold $\esafe$, we can control the amount of risk taken by the agent.}
    \vspace{-0.2cm}
    \label{fig:drunkspider}
\end{wrapfigure}

To answer question (3), we now aim to assess the stability and efficiency of learning when using the safety-critic. To do so, we present learning curves for SQRL and our comparisons in Figures~\ref{fig:safety_stability} and~\ref{fig:cumulative_failures} (in Appendix~\ref{appendix:training-plots}). In these curves, we find that SQRL not only reduces the chances of safety incidents (Figure~\ref{fig:cumulative_failures}), but also significantly speeds up and stabilizes the learning process (Figure~\ref{fig:safety_stability}). In particular, we observe large performance drops during SAC training, primarily due to exploration of new policies, some of which are unsafe and lead to early termination and low reward. Our approach instead mitigates these issues by exploring largely in the space of safe behaviors, producing more stable and efficient learning. We also show that when fine-tuning for the cube rotation task, the safety policy can be overly cautious (see Figures~\ref{fig:safety_stability} and~\ref{fig:cumulative_failures} in the appendix), resulting in fewer failures but lower performance than the unconstrained SAC policy. These results indicate that even when the fine-tuning task is a more difficult version of the original training task, a task-agnostic safety Q-function can guide exploration to be safer while learning to solve the new task. 

% Additionally

%As a worthwhile next step, this ability to bootstrap and generalize from previously learned safety-models could potentially be used in a curriculum that gradually teaches the robot to move faster and faster, while restricting the danger of falling at high speeds.

%These performance drops during learning for SAC are primarily due to exploring new policies that are unsafe and lead to shorter episodes, which our method naturally mitigates, focusing only on collecting experience that will help it solve the task more quickly.


%In addressing question (3), the performance of our trained agent during fine-tuning is largely affected by how often it must reset while learning, since in order to continue learning to manipulate a cube or walk faster, it must ensure that the cube is in hand, or that the robot is still standing up. Using the safety-critic to avoid early termination therefore has the benefit of stabilizing learning by making it easier for the agent to only explore actions that allow it to stay alive longer in an episode while attempting to maximize reward. 

%This is clear when seeing that SQRL both (a) outperforms the other methods in terms of failure rate (see~\ref{fig:bar-plot}), and (b) has a smoother learning curve during pre-training and fine-tuning that does not drop significantly in performance over the course of learning (see~\ref{fig:learning-curves}).

%With the simple addition of learning exploration constraints from resets that reject unsafe actions, our method simplifies the burden of designing a reward function to encourage task success while discouraging unsafe behaviors, and shows that using simple binary safety labels is sufficient to avoid unsafe states during training.  
%Looking at the cumulative regret curves and failure rates between fine-tuning the SAC pre-trained policy and the SQRL pre-trained policies (Fig.~\ref{fig:mini-curves}), we show that our model reaches the goal speed faster with fewer failures than the baseline. This indicates that even when the fine-tuning task is a more difficult version of the original training task, a task-agnostic safety Q-function can guide exploration to be safer while learning to solve the new task. As a worthwhile next step, this ability to bootstrap and generalize from previously learned safety-models could potentially be used in a curriculum that gradually teaches the robot to move faster and faster, while restricting the danger of falling at high speeds.


% \todo{talk about affect on stability}

\subsection{Trading Off Risk and Reward with $\esafe$}

% \begin{figure}
%     \vspace{-0.2cm}
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figures/safe-vs-risky.pdf}
%      \vspace{-0.2cm}
%     \caption{Qualitative results showing different trajectories corresponding to different target safety thresholds. By tuning the safety threshold $\esafe$, we can control the amount of risk taken by the agent.}
%     \label{fig:drunkspider}
%     % \vspace{-2em}
% \end{figure}


\iffalse
\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{Figures/mini-pretrain-stable.pdf}
    \caption{Pre-training learning curves for the MinitaurVelocity and Cube environments that show stable learning during pre-training for an optimistic ($\esafe=0.15$) and pessimistic ($\esafe=0.05$) safety-critic, compared with SAC.}
    \label{fig:learning-curves}
\end{figure}
\fi




% \begin{figure}
%     \begin{subfigure}[b]{.49\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm]{Figures/num-resets.pdf} % cum-fail-mini.pdf
%         % \caption{Final / maximum possible reward}
%         \caption{Cumulative failures during fine-tuning}
%         \label{fig:min-vel-num-resets}
%     \end{subfigure}
%     \begin{subfigure}[b]{.49\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm]{Figures/min-vel-ret-ft.pdf}
%         \caption{Fine-tuning learning curves}
%         \label{fig:min-vel-ret-ft}
%     \end{subfigure}
%     \caption{Learning and cumulative failure curves for pre-training on Minitaur Velocity task.}
%     \label{fig:mini-curves}

% \end{figure}

%\todo{this subsection needs to be revised to discuss drunk spider env}

Finally, we aim to answer question (4). We aim to evaluate whether the safety threshold, $\esafe$, can be used to control the amount of risk the agent is willing to take. To do so, we consider the drunk spider environment, evaluating two different values of our safety threshold, $\esafe=0.2$ and $\esafe=0.05$, with action noise included in the environment with magnitude $\varepsilon_\text{action}=0.2$. In Figure~\ref{fig:drunkspider}, we observe that, when using the conservative safety threshold of $\esafe=0.05$, the agent chooses to cautiously move around the two pits of lava, taking the long but very safe path to the goal location in green. Further, when we increase the safety threshold to a maximum failure probability of $\esafe=0.2$, we find that the agent is willing to take a risk by navigating directly through the two pits of lava, despite the action noise persistent in the environment. We observe that these two behaviors are consistent across multiple trials. Overall, this experiment suggests that tuning the safety threshold $\esafe$ does provide a means to control the amount of risk the agent is willing to take, which in turn corresponds to the value of the task reward and efficiency relative to the (negative) value of failure. This knob is important for practical applications where failures have varying costs.

%We test whether the safety-critic's threshold can be used to control how risk-averse or risk-seeking the agent learns to behave in the cube rotate environment. As shown in Figure~\ref{fig:safety-thresh}, our results showed that varying $\esafe$ can trade safety for final performance. This gives a new interpretable control knob for maximum-entropy reinforcement learning, which would otherwise be difficult to tune to satisfy different degrees of safety requirements.






%\paragraph{Drunk Spider}
%The drunk spider environment is a 2D navigation environment, where the agent must learn to navigate from the start to a fixed goal position, in a continuous state and action space. The drunk spider environment adds the difficulty of creating a narrow bridge that goes directly from start to goal, with two lava pits on either side which terminate the episode if the agent falls into either one. Additionally, if the agent is unconfident about crossing the bridge without falling, it can instead choose to go around the bridge and lava pits entirely, which takes longer (\textit{i.e.}, costs more) but avoids the risk of falling into the lava.

%In our experiments, we train and evaluate our method using a set of tasks which involve varying amounts of noise added to the actions taken by the agent, making it in some cases too difficult to cross the bridge without some probability of falling off. This encourages the policy to learn both strategies of reaching the goal, depending on the amount of noise added.



% TABLE MOVED TO FIGURE (BAR PLOT) BELOW 
% \begin{table}[t]
% \caption{(Total of Maximum Reward \%, Total Failure Rate \%) fine-tuning results 
% compared for the point-mass, minitaur, and cube-rotation environments.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Task & SQRL (ours)  & SAC (pre-trained) & SAC (from scratch) & Ensemble-SAC & WCPG  \\
% \midrule
% Drunk-Spider        &(97\%, 1\%) & (91\%, 17\%) & (90\%, 24\%) & () & (92\%, 20\%) \\
% Minitaur-Friction   &()       &()       &()       &()       &() \\
% Minitaur-Velocity   &(67\%, 6\%) & (73\%, 17\%) & (76\%, 27\%) & () &(29\%, 15\%) \\
% Cube-Rotation       &(59\%, 14\%)& (70\%, 19\%) & ()       &()       &(53\%, 33\%) \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


\iffalse
%% Omitting this.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{Figures/final-cube-rew-fail.png}  % Shows regret as fraction of # missed steps due to reset / total steps trained
    %%BE.2.4: Is there a reason to use neg distance from goal instead of dist from goal? I don't understand what the X axis indicates. Can we somehow get more dots on this plot? For example, we could plot the performance of checkpoints/iterates during training.
    \caption{Trade-offs between safety and total reward for the Cube Rotate task (``eps'' is the target safety value $\esafe$), showing how the safety threshold affects the tradeoff between safety-regret and reward. Regret is measured as number of total missed opportunities for reward as a percentage of the total steps.} % failure / # timestepsI
    %%BE.2.4: One thing to think about is that many readers, including the reviewers, will start by just reading the figures and captions. It's great if the figures by themselves can convey what the main idea of the paper is. Of course, it's often challenging to do this in a concise way. If nothing else, we should include a sentence in most figure telling the reader what they are supposed to learn. For example, "[desribe what we're plotting, what the axes are, etc]. We observe that SQRL achieves a larger reward with a fewer number of failues, and the safety threshold controls the tradeoff between safety and reward."
    % \vspace{-5mm}
    \label{fig:safety-thresh}
\end{figure}
\fi

%\subsection{Varying Safety Threshold}



% \subsection{Effect on Pre-Training and Fine-tuning Performance}

% \todo{merge any content in this section with the above subsections, and remove this one.}

% \begin{figure}[b!]
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth]{ds-avg-ret} 
% \caption{Drunk spider environment average return}
% \label{fig:ds-avgret}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth]{ds-ep-succ}
% \caption{Drunk spider environment episode success}
% \label{fig:ds-epsucc}
% \end{subfigure}
% \caption{Comparison of baselines and our work on drunk spider environment, averaged over 5 seeds}
% \label{fig:ds-baselines}
% \end{figure}

% In addition to showing that how our method could be used to control emergent policy behavior, we also compared our pre-training and fine-tuning training performance to other methods on more quantitative metrics and noted several advantages to using our approach.

% TODO : adding fine-tuning training curves for minitaur
% \begin{figure}[t!]
%     \centering
    % \includegraphics[width=0.75\linewidth]{minitaur-safety}
%     \caption{Minitaur pre-training and fine-tuning performance, compared with SAC}
%     \label{fig:minitaur-safe}
% \end{figure}

% One striking result in both drunk spider and Minitaur environments is how the use of the task-agnostic safety labels to condition the policy to mask out ``unsafe'' actions guides the exploration to converge to an optimal policy in fewer steps than learning without these additional safety signals (\textit{i.e.}, only using negative rewards). With the simple addition of learning exploration constraints from resets, our method simplifies the burden of designing a reward function to encourage task success while discouraging unsafe behaviors, and shows that using simple binary safety labels is sufficient to avoid unsafe states during training. 

% In fine-tuning on the minitaur locomotion task, our method succeeded in getting the robot to learn to walk at a faster speed (from 0.3 to 0.5 m/s) without falling as often as SAC or WCPG. Looking at the cumulative regret curves and failure rates between fine-tuning the SAC pre-trained policy and the SQRL pre-trained policies (Fig.~\ref{fig:mini-curves}), we show that our model reaches the goal speed faster with fewer failures than the baseline. This indicates that even when the fine-tuning task is a more difficult version of the original training task, a task-agnostic safety Q-function can guide exploration to be safer while learning to solve the new task. This ability to bootstrap and generalize from previously learned safety-models could potentially be used in a curriculum that gradually teaches the robot to move faster and faster, while restricting the danger of falling at high speeds.

==> Learning to be Safe - Arxiv/7-conclusion.tex <==
%%CF.2.2: Here's how I might suggest writing the conclusion:
We introduced an approach for learning to be safe and then using the learned safety precautions to act safely while learning new tasks. Our approach trains a safety-critic to estimate the probability of failure in the future from a given state and action, which we can learn with dynamic programming. We impose safety by constraining the actions of future policies to limit the probability of failures. Our approach naturally yields guarantees of safety under standard assumptions, and can be combined in practice with expressive deep reinforcement learning methods. On a series of challenging control problems, our approach encounters substantially fewer failures during the learning process than prior methods, and even produces superior task performance on one task.

Our experimental results make strides towards increasing the safety of learning, compared to multiple prior methods.
However, there are a number of potential avenues for future work, such as optimizing the pre-training or curriculum generation procedures.
Relaxing some of the assumptions to guarantee that a constrained policy is safe may yield alternative ways of calculating risk and sampling safe actions under the Q-learning framework we propose.
Motivated by our analysis, another area for study is handling out-of-distribution queries to the safety-critic. 
% more exploratory pre-training, a finer curriculum, or motivated by our analysis, incorporating general constraints on state-action pairs in which the safety-critic is queried to prevent out-of-distribution queries. 
Finally, encouraged by the strong results in simulation, we aim to apply SQRL to real-world manipulation tasks in future work.
% Nonetheless, given the promising results in simulated control tasks, experimenting with more realistic tasks such as those on robotic hardware is an exciting direction for future investigation.


\iffalse
We introduced a novel addition to the SAC algorithm that uses binary reward signals to learn a task-agnostic safety-critic that can be used to learn safely. In our experiments on the drunk spider point-mass and Minitaur quadrupedal locomotion environments, we showed that our method outperforms similar baselines that do not utilize safety models, and can lead to better pre-training and fine-tuning performance on these environments.  One interesting outcome of this work is that the safety-threshold term used by the safety-critic can influence the policy behavior to be either more or less risk-averse, allowing the user to control how safely the robot explores the environment. For instance, in the drunk spider environment, this corresponded to whether the policy chose to go through a narrow corridor to reach the goal state, where it could potentially fall into a lava pit, or whether it chose to go around the pit to reach the goal.

Our algorithm also demonstrates benefits in fine-tuning performance. For example, in the Minitaur environment, we show how the robot could learn to move faster without falling by using the pre-trained policy and safety-critic. This is intuitive given that a reasonable curriculum for learning to walk faster would be to begin with learning to walk slowly without falling down, then eventually increase the speed.

In this work, we have primarily looked at the multi-task setting with a curriculum for learning to perform more difficult tasks. For future directions, it would be useful to see whether training the safety-critic on more tasks makes it forget how to be safe in earlier seen tasks, and evaluate if it can be trained to be invariant not only to the task but the policy being used as well. Lastly, it would be worth exploring if it is possible to tune $\gsafe$, which controls the safety window at the end of the trajectory, adaptively, rather than needing to set it explicitly as a hyperparameter.
%%CF.2.2: These sorts of details are better left for the appendix.
\fi

%%CF: I'm commenting this out for the arxiv version
\iffalse
\section*{Broader Impact}
% Safety guarantees are a necessary component of robot learning algorithms in order for general-purpose robots to come more widely into use in human environments.
Safety guarantees are a necessary component for deploying general-purpose robots into environments with humans.
As the RL and robotics communities move towards learning-based approaches, we believe that incorporation a notion of safety into the learning process will become increasingly important.
We highlight two potential broader impacts of this work. First, and most immediately, the safety model that we learn has the potential to reduce the risk of catastrophic failures when deploying robots in the real world. Second, and slightly more abstractly, while there are many ways to imbue a sense of safety into an intelligent agent, we broadly advocate for a learned notion of safety. We expect that learned approaches to safety will be easier to build and apply to high-dimensional tasks, especially those settings where manual reward design is challenging and human supervision is expensive.

We highlight three potential risks with our approach, relating to collecting a dataset of failures, balancing false positives and false negatives, and adversarial examples.
One major challenge with our approach to safety is collecting a diverse and realistic dataset of failures without endangering people and property. 
% While simulators continue to improve, they mayalso influence the bias and blindspots of a model that is trained without real-world experience.
While simulators continue to improve, they will remain \emph{approximate} models of the world. Human designers of simulators are likely to spend their engineering efforts on improving simulation of ``normal'' behavior, so the simulation of failure cases may be less precise.
A second challenge lies in the automatic detection of failures. Both false positive and false negatives are problematic. For example, in a self-driving car, a false positive could result in suddenly applying the brakes due to a phantom obstacle; a false negative could result in failing to apply brakes before a real obstacle.
Third, our method is also subject to existing challenges in adversarial robustness among learning-based methods~\cite{goodfellow2014explaining}. In our approach, the policy may attempt to find actions that that safety-critic mistakenly thinks are safe. Augmenting our safety-critic with adversarial robustness techniques~\cite{engstrom2019adversarial} could mitigate against this risk.
\fi

==> Learning to be Safe - Arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\todo}[1]{\cmt{TO-DO: #1}}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Safety critic
\newcommand{\qsafe}{\ensuremath{Q_{\text{safe}}}}
\newcommand{\esafe}{\ensuremath{\epsilon_\text{safe}}}
\newcommand{\gsafe}{\ensuremath{\gamma_\text{safe}}}
\newcommand{\pisafe}{\ensuremath{\pi^\text{safe}}}
\newcommand{\sunsafe}{\ensuremath{\mathcal{S}_{\text{unsafe}}}}
\newcommand{\ptask}{\ensuremath{\gT_\text{pre}}}
\newcommand{\gtask}{\ensuremath{\gT_{\text{target}}}}
